Very accurate time propagation of coupled Schr\"odinger equations for femto- and attosecond physics and chemistry, with C++ source code

In this article, I present a very fast and high-precision (up to 33 decimal places) C++ implementation of the semi-global time propagation algorithm for a system of coupled Schr\"odinger equations with a time-dependent Hamiltonian. It can be used to describe time-dependent processes in molecular systems after excitation by femto- and attosecond laser pulses. It also works with an arbitrary user supplied Hamiltonian and can be used for nonlinear problems. The semi-global algorithm is briefly presented, the C++ implementation is described and five sample simulations are shown. The accompanying C++ source code package is included. The high precision benchmark (long double and float128) shows the estimated calculation costs. The presented method turns out to be faster and more accurate than the global Chebyshev propagator.

==> makefile <==
# .PHONY to są te które zawsze się wykonują, bez komunikatu "target is up to date"
.PHONY: markdown_test reviewers_response

all:
	pdflatex manuscript.tex && bibtex manuscript && pdflatex manuscript.tex && pdflatex manuscript.tex

clean:
	rm -f manuscript.aux manuscript.bbl manuscript.blg manuscript.log manuscript.spl manuscript.out
#Przycinanie .eps do .pdf
# ps2pdf -dPDFSETTINGS=/prepress -dEPSCrop file.eps

watchCompile:
	while true;do ./sh_last_change.sh || /usr/bin/time -f "\n\twall clock time: %E" make warn; sleep 1; done

warn:
	${MAKE} all 2>&1 | grep -v fancyhdr | grep -v hyperref | grep --color=always -iE "error:|warning|^l\..*" -A 3 -B 1 || true
	touch /tmp/last16-Schaefer2017-CPP_make

response2:
	pandoc -V geometry:margin=25mm -V colorlinks=true -V linkcolor=blue -V urlcolor=blue -V toccolor=gray -V fontsize=11pt -o ./v2-submitted/submitted/response.pdf ./v2-submitted/submitted/response.md
	#pandoc -V geometry:margin=25mm -V colorlinks=true -V linkcolor=blue -V urlcolor=blue -V toccolor=gray -V fontsize=11pt -o ./v2-submitted/submitted/CRediT.pdf ./v2-submitted/submitted/CRediT.md

reviewers_response:
	pandoc -V colorlinks=true -V linkcolor=blue -V urlcolor=blue -V toccolor=gray -V papersize:a4 --pdf-engine=xelatex --filter=pandoc-citeproc -o ./v3-submitted/submitted/reviewers_response.pdf ./v3-submitted/submitted/reviewers_response.md

markdown_test:
	pandoc -V geometry:margin=25mm -V colorlinks=true -V linkcolor=blue -V urlcolor=blue -V toccolor=gray -V fontsize=11pt -o ./markdown_test/markdown_test.pdf ./markdown_test/markdown_test.md

